A Scalable Concurrent Algorithm for Dynamic Connectivity

Dynamic Connectivity is a fundamental algorithmic graph problem, motivated by a wide range of applications to social and communication networks and used as a building block in various other algorithms, such as the bi-connectivity and the dynamic minimal spanning tree problems. In brief, we wish to maintain the connected components of the graph under dynamic edge insertions and deletions. In the sequential case, the problem has been well-studied from both theoretical and practical perspectives. However, much less is known about efficient concurrent solutions to this problem. This is the gap we address in this paper. We start from one of the classic data structures used to solve this problem, the Euler Tour Tree. Our first contribution is a non-blocking single-writer implementation of it. We leverage this data structure to obtain the first truly concurrent generalization of dynamic connectivity, which preserves the time complexity of its sequential counterpart, but is also scalable in practice. To achieve this, we rely on three main techniques. The first is to ensure that connectivity queries, which usually dominate real-world workloads, are non-blocking. The second non-trivial technique expands the above idea by making all queries that do not change the connectivity structure non-blocking. The third ingredient is applying fine-grained locking for updating the connected components, which allows operations on disjoint components to occur in parallel. We evaluate the resulting algorithm on various workloads, executing on both real and synthetic graphs. The results show the efficiency of each of the proposed optimizations; the most efficient variant improves the performance of a coarse-grained based implementation on realistic scenarios up to 6x on average and up to 30x when connectivity queries dominate.

==> [SPAA] Concurrent Dynamic Connectivity Online (1)/connected.tex <==
  \begin{lstlisting}
func connected(u, v: Vertex): Bool = while (true) {
  // Get the roots of `u` and `v` with the versions
  (u_root, u_version) := find_root(u)
  (v_root, v_version) := find_root(v)
   // Has the component of `u` been changed?
  if (u_root, u_version) != find_root(u): continue
  if u_root != v_root: 
  #\indentrule#  // `u` and `v` are likely to be in different 
  #\indentrule#  // components, re-check that `u_root` and
  #\indentrule#  // `v_root` were snapshotted atomically
  #\indentrule#  if (v_root, v_version) != find_root(v): continue    
  #\indentrule#  if (u_root, u_version) != find_root(u): continue#\label{line:connected:last_search}#
  return u_root == v_root
} 
// Returns the root with the current version
func find_root(u: Vertex): (Vertex, Int) {
  cur := u
  while (true):
  #\indentrule#  parent := cur.parent // read the parent of `cur`
  #\indentrule#  if parent == null: break // is `cur` the root?
  #\indentrule#  cur = parent // go towards the root
  // Return the found root with the current version
  return (cur, cur.version)
}
  \end{lstlisting}

